Physically Grounded Monocular Depth via Nanophotonic Wavefront Encoding

Depth foundation models (DFMs) offer strong learned priors for 3D perception from single RGB images but lack physical depth cues, leading to ambiguities in metric scale. We introduce metalenses, an emerging class of ultrathin planar optical elements, as a solution to physically encode missing metric depth cues via nanophotonics. In this paper, we bridge the gap between metalens and DFMs to achieve accurate metric monocular depth sensing. In a single monocular shot, our metalens embeds depth-dependent positional shifts into two polarized optical wavefronts. With an input adaptation strategty, we enable direct fine-tuning that aligns a pretrained DFM with the optical signals. To scale the training data, we further develop a comprehensive simulation pipeline that synthesizes metalens responses from RGB-D datasets, incorporating physical factors to minimize the sim-to-real gap. Experiments demonstrate that this approach outperforms both monocular metric depth estimation and depth-from-defocus baselines, showing an effective pathway for accurate monocular metric depth sensing.

==> tools/package.tex <==
% Commonly used abbreviations (\eg, \ie, \etc, \cf, \etal, etc.)
\usepackage{eccvabbrv}

% The "axessiblity" package can be found at: https://ctan.org/pkg/axessibility?lang=en
\usepackage[accsupp]{axessibility}  % Improves PDF readability for those with disabilities.

%%% Language %%%%
\RequirePackage[english]{babel}                  % Hyphenation and date format
\RequirePackage{xspace}                          % Abbreviation spacing
\RequirePackage{xpunctuate}                      % Abbreviation spacing

%%% Tex-scripting %%%
\RequirePackage{ifthen}                          % If-then-else latex logic
\RequirePackage{soul}                            % Underlining and Strike-through
\RequirePackage{xargs}                           % For \newcommandx

%%% Color %%%
\RequirePackage{color}                           % Draft annotation coloring
\usepackage{xcolor}
\usepackage[table]{xcolor}

%%% Math-mode %%%
\RequirePackage{amsmath}                         % Math equations
\RequirePackage{bm}                              % Math bold symbols

%%% Cross-referencing %%%
%\RequirePackage[toc,page,titletoc]{appendix}     % Appendix section
%\RequirePackage[capitalize,nameinlink]{cleveref} % Easy to use cross-referencing
% \crefname{supp}{Supplement}{Supplements}     % Supplement section name setting

%%% Figures %%%
% \RequirePackage{caption}                         % Figure captions
% \RequirePackage{subcaption}    
% \RequirePackage{subfig}                          % Nested figures

%\usepackage{accents}
\usepackage{float}
\usepackage{multirow}  % put this in your preamble
\usepackage{makecell}

\usepackage{tikz}
\usetikzlibrary{backgrounds}
\usepackage{diagbox}
\usepackage{adjustbox}
\usepackage{stfloats}   % in preamble
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{graphicx}
\usepackage{amssymb}
\usepackage{booktabs}

\usepackage{hyperref}


% Support for ORCID icon
\usepackage{orcidlink}

% \usepackage{alltt}
% \usepackage{amsthm}
% \usepackage{newlfont}
% \usepackage{floatflt}
\usepackage{wrapfig}
% \usepackage{fixltx2e}
% \usepackage{multirow}
% %\usepackage{cleveref}
% \usepackage{algorithmic}
% \usepackage[export]{adjustbox}
% \usepackage{mathtools, cuted}
% \usepackage{CJKutf8}
% \usepackage[toc,page,titletoc]{appendix}
% \usepackage[ruled]{algorithm2e}
% \usepackage{enumitem}
% \usepackage{harpoon}
\usepackage{esvect}

